Identifying Driver Interactions via Conditional Behavior Prediction

Interactive driving scenarios, such as lane changes, merges and unprotected turns, are some of the most challenging situations for autonomous driving. Planning in interactive scenarios requires accurately modeling the reactions of other agents to different future actions of the ego agent. We develop end-to-end models for conditional behavior prediction (CBP) that take as an input a query future trajectory for an ego-agent, and predict distributions over future trajectories for other agents conditioned on the query. Leveraging such a model, we develop a general-purpose agent interactivity score derived from probabilistic first principles. The interactivity score allows us to find interesting interactive scenarios for training and evaluating behavior prediction models. We further demonstrate that the proposed score is effective for agent prioritization under computational budget constraints.

==> EXTERNAL_ Identifying Driver Interactions via Conditional Behavior Prediction/deprecated/notes2.tex <==
Summary:
TODO 0) Trim to 6 pages + references. How?
TODO - 1) Action item: qualify the CBP contribution
Bala is working on experiments -> 2) Action item: show that our model is SOTA, as one of its contributions
Done -> 3) Action item: use influencer/follower in the motivation as an example, but not everywhere after. 

Detailed comments and misc edits below:

Compare to other CBP methods: Dorsa Sadigh introduced the idea in RSS’16 (with IRL-based models), and Ed Schmerling did it with neural nets (conditional VAEs) in ICRA’18. 

Explain surprise in more detail.  One section claims that it predicts “surprise”, meaning situations where marginal predictions are different from conditional predictions. It does so by definition. Why is that useful though? 

Explain that the "Selecting Salient Agents" section is actually imitating a planner, so we are demonstrating what's useful for a planner. 
To show utility, you’d have to actually use these in planning and show that ignoring the agents with low mutual information does not affect the AV’s performance (either the plan, or, more ideally, the cost/reward of the resulting behavior when the ignored agents are actually present). 

Explain why we don't use joint models P(a,b), rather than having to train a conditional prediction model P(b|a). How can you justify conditional prediction? 

Results comments:

B is more of a sanity check that conditioning is helpful; Early fusion vs late fusion stuff — seems tangential/ distracts from the point 

C what’s the takeaway? Is this useful or purely informational or a sanity check on the score?

D 

Not sure what the term surprise refers to here, and what “surprising” interactions are. We throw it around at waymo but it’s not established in the robotics, HRI, and ML literature. It seems to be defined as KL divergence being high :)

Fig 4a the fact that what has highest mutual information has low to lowest delta wade, explained in the text as wade not being meaningful, seems to somewhat invalidate using it as a way to sanity check the score. 

4b seems to indicate that maybe the paper should have been about the KL divergence as a metric, or at least in equal parts with info gain. But the fact that it doesn’t have the problem that 4a has suggests that perhaps there is something wrong with Info gain not actually pointing at the kind of interactivity we care about.

E not sure how all of the sudden there is an AV, as the dataset described in the beginning mentioned “agents” (btw, waymo refers to humans as agents, but it’s not standard) — was there an AV in the data all along? Did it drive in manual? 

Need to motivate why you’d ignore agents for planning.

Other:

Need to change to active voice — you’re using passive voice too much which leads to reader fatigue.

==> EXTERNAL_ Identifying Driver Interactions via Conditional Behavior Prediction/deprecated/old_intro.tex <==
% MOVE TO RELWORK:
% Clearly, obtaining accurate predictions for other agents requires accounting for their interactions. There are a variety of existing approaches which attempt to do this task using relationship-based deep learning architectures such as transformers \cite{giuliari2020transformer}, or Graph Neural Networks (GNNs) \cite{casas2019spatially}, with positive results. 

% However, the field currently lacks a rigorous mathematical treatment of the notion of an interaction. We define interactions in the context of behavior prediction via an information-theoretic approach, and show how this treatment can provide key benefits when constructing behavior prediction models. 
% \textcolor{red}{Mathematical Details}
% Specifically, we use the \emph{mutual information} between the future trajectories of a pair of agents as an interactivity score that represents the potential for the two agents to have an unexpected interaction. %To compute an estimate of the mutual information between agent trajectories, we leverage state of the art BP models.


% \textcolor{red}{CBP}
% One important outcome of this work is the notion of a \emph{Conditional Behavior Prediction (CBP)} model. Typical behavior prediction systems are unconditional, and their outputs do not take the AV's plan into account \cite{bajcsy2020}. This imposes certain limitations on the system, as it encodes the assumption that human-driven cars will not react to the autonomous vehicle, often resulting in overly-cautious behaviors \cite{fisac2018probabilistically}. We leverage our work on interactions to develop a new approach to behavior prediction where predictions are conditioned on the planned trajectory of the AV.  
% We show that modeling the potential effect of the AV's behavior on other agents can greatly improve prediction accuracy, resulting in faster and safer AV behavior.


% \textcolor{red}{Importance of Autonomous driving}
% Autonomous driving is a key area of active research in the machine learning community. Autonomous vehicles have the potential to prevent accidents, save lives, reduce congestion, and empower those who are unable to drive themselves. It is also considered a gateway technology to the development of more general autonomous agents which can function freely within a chaotic human world. 
% %Most autonomous driving systems can be decomposed into three distinct components: Perception, Behavior Prediction, and Planning. Perception resolves sensor data into objects, BP predicts the future location of dynamic objects, and planner uses these predictions as constraints to chart a course for the AV.

% \textcolor{red}{Behavior Prediction }
% Behavior Prediction (BP) is a core component in modern AV systems. BP is the process of mapping past observations to a distribution over possible future agent trajectories. These predictions are crucial when creating a motion plan for the AV. BP is a complex and challenging task, as it requires jointly modelling a collection of unique human agents with unknown intent. Furthermore agent behavior is highly interactive, with each agent continuously modulating its actions based on the observed behavior of those around it. 

% \textcolor{red}{Importance of interactions}
% It is clear that obtaining accurate BPs requires us to account for these interactions in our model. There are a variety of existing approaches which attempt to do this using relationship-based deep learning architectures such as transformers or GNNs \cite{casas2019spatially, giuliari2020transformer}, with positive results. However, the field currently lacks a rigorous mathematical treatment of the notion of an interaction. We define interactions in the context of BP via an information theoretic approach, and show how these results can provide key benefits when constructing BP models. 
% \textcolor{red}{Mathematical Details}
% Specifically, we use the mutual information between the future trajectories of a pair of agents as an interactivity score that represents the potential of two agents to have a surprising interaction. %To compute an estimate of the mutual information between agent trajectories, we leverage state of the art BP models.

% \textcolor{red}{CBP}
% In particular, one important outcome of this work is the notion of a conditional behavior prediction model. Existing BP systems are unconditional, with the predicted behavior static during the planning phase \cite{bajcsy2020}. This imposes certain limitations on the system, as it encodes the assumption that human-driven cars will not react to the autonomous vehicle, often resulting in overly cautious behaviors \cite{fisac2018probabilistically}. We leverage our work on interactions to develop a new approach to BP where predictions are conditioned on the planned trajectory of the AV. We call this approach \emph{Conditional} behavior prediction (CBP). We show that predicting the effect of AV motion on agent behavior can greatly improve predictive accuracy, resulting in faster and safer AV behavior.

% \textcolor{red}{contributions}
% Our contributions can be summarized as follows: (1) We provide a problem-agnostic definition of agent interaction and a quantitative interactivity score. (2) We propose a unified architecture for conditional behavior prediction. (3) We demonstrate the utility of identifying interactions in real traffic scenarios.


%In traditional behavior prediction we estimate a distribution over future trajectories for each agent independently. This means that when we consider multiple agents in a scene, their BPs are often conflicting or inconsistent. More advanced approaches attempt to produce joint predictions which produce consistent predictions for all agents in a scene using models such as transformers or graph neural networks. We propose taking this a step further and conditioning our predictions 

%\textcolor{red}{Importance of CBP}
% On the road, an autonomous vehicle's action can affect the actions of other cars. Robot motion planning in the presence of humans is a well studied challenge.  Most planning approaches assume that human-driven cars will not react to the autonomous vehicle, often resulting in overly cautious behaviors \cite{fisac2018probabilistically}. Others approaches focus on planning using a cost function that combines efficiency of the trajectory and the inferred cost functions of human drivers \cite{sadigh2016planning}. In challenging scenarios, the autonomous car may need to balance the influence on other drivers with efficiency objectives. Predicting the effect of potential future plans on others can allow a planner to perform these trade-offs explicitly and make the resulting trajectories more efficient and safe.

% Another application could be focusing only on salient agents when simulating reactive policies for testing autonomous driving software.
% \textcolor{red}{Motivation 1) Anticipating situations of surprise. 2) Identifying interacting agents for high-fidelity prediction models/planning.}

% Interactive driving scenarios, such as lane changes, merges or unprotected turns, are some of the most challenging problems for autonomous driving. Planning in interactive scenarios requires accurately predicting the reactions of other agents to a particular future action. We develop end-to-end models for conditional behavior prediction (CBP) that take as an input a potential future trajectory for a vehicle, and predict the effect of this trajectory on other vehicles in the scene. 

%\textcolor{blue}{multi-modality of predictions, why MultiPath}
%A major challenge in driver behavior prediction is the inability to observe an agent's intention or goal. As a result, a drivers' behavior may appear multi-modal, with several possible actions being equally likely. We use the MultiPath architecture that explicitly predicts multi-modal distributions for the future trajectories of each agent \cite{chai2019multipath}.
%MultiPath is a one-shot long-horizon model so it allows us to capture longer-term correlations between agents’ futures. The interactivity score between two agents over a single time-step may be small, but only using one-shot long-horizon prediction models can we draw a more definitive conclusion. The long-horizon model also can capture second order effects in which the actions of one agent cause a chain reaction of influence, like sudden braking propagating several cars back. Therefore, the Conditional MultiPath \textcolor{red}{Let's define this properly first} model is unique in its ability to identify interactive situations. 



%\textcolor{blue}{related work in CBP/joint prediction}
%What-If Motion Prediction predicts the future trajectory for an agent conditioned on its nominal desired future trajectory \cite{khandelwal2020if}. Conditional MultiPath is not unique in its ability to perform multi-modal multi-agent behavior prediction, but it is uniquely suited for the use of its outputs for further analysis of driver interaction.


% Several state-of-the-art behavior prediction approaches also provide the ability to evaluate joint futures of multiple vehicles \cite{tang2019multiple, rhinehart2019precog, salzmann2020trajectron++, mangalam2020not, khandelwal2020if}. Like Conditional MultiPath, several other architectures allow the evaluation of conditional futures for a particular plan of the autonomous car. The Multiple Futures Prediction approach computes joint behavior predictions for multiple agents and also provides the ability to do hypothetical rollouts, but only limited evaluation is performed for this feature \cite{tang2019multiple}. PRECOG  provides a conditional query to the model via a latent space \cite{rhinehart2019precog}. The system must optimize over the latent vector to find the desired trajectory closest to the plan of the autonomous vehicle. Trajectron++ demonstrates the use of the ego future for improving behavior metrics on average, but does not consider conditioning on other vehicles \cite{salzmann2020trajectron++}. PECNet  infers possible goal locations for other agents and uses those to perform more accurate behavior prediction \cite{mangalam2020not}.



% \textcolor{blue}{The story from delta log likelihood, to KL divergence, to mutual information goes here.}



%\cite{kruse2013human}
% \textcolor{red}{Importance of Autonomous driving}
% Autonomous Vehicles (AVs) have the potential to prevent accidents, save lives, reduce congestion, and empower those who are unable to drive themselves. Autonomous driving is a key area of active research in the machine learning community and a gateway technology to the development of more general autonomous agents, which can function freely within a chaotic human world. 
%Most autonomous driving systems can be decomposed into three distinct components: Perception, Behavior Prediction, and Planning. Perception resolves sensor data into objects, BP predicts the future location of dynamic objects, and planner uses these predictions as constraints to chart a course for the AV.

% Another body of work seeks to learn a reward function of human agents via inverse reinforcement learning and use this reward to plan robot trajectories that optimize for both the robot's and humans objective \cite{ziebart2009planning, sadigh2016planning}. Recent work in the field seeks to predict the future trajectory of a human agent in proximity of a robot, and constrain the planning problem based on the predicted dynamic occupancy \cite{fisac2018probabilistically}. A Bayesian model of the future trajectory can allow the robot to plan more aggressive trajectories when the prediction uncertainty is low \cite{bajcsy2019scalable}. The predictions may be inaccurate if the intent of the human agent is unknown, so the robot may need to be robust to any possible future human trajectory \cite{bajcsy2020}. %Another work seeks to model the trajectories of the human and robot as Gaussian Processes and the model can be conditioned on the goal pose of the robot \cite{trautman2010unfreezing}.

% The biggest limitation of many of the approaches mentioned for human-aware control is the simplicity of the behavior prediction model. Real road traffic scenarios can include challenging interactions among dozens of agents, such as drivers, cyclists and pedestrians, and the problem of driver behavior prediction is an emerging field of research. Several state-of-the-art behavior prediction approaches provide the ability to evaluate joint futures of multiple vehicles \cite{tang2019multiple, rhinehart2019precog, salzmann2020trajectron++, mangalam2020not, khandelwal2020if}. Furthermore, several of these architectures allow the evaluation of conditional futures for a particular plan of the autonomous car. The Multiple Futures Prediction approach computes joint behavior predictions for multiple agents and also provides the ability to do hypothetical rollouts, but only limited evaluation is performed for this feature \cite{tang2019multiple}. PRECOG  provides a potential future AV trajectory to the model via a latent space representation \cite{rhinehart2019precog}. The system must optimize over the latent vector to find the desired trajectory closest to the plan of the autonomous vehicle. Trajectron++ demonstrates the use of the ego future for improving behavior metrics on average, but does not consider conditioning on other vehicles \cite{salzmann2020trajectron++}. PECNet infers possible goal locations for other agents and uses those to perform more accurate behavior prediction \cite{mangalam2020not}.
% Our approach to estimating agent interactivity scores could potentially be used with any model that enables the evaluation of conditional predictions.





==> deprecated/notes2.tex <==
Summary:
TODO 0) Trim to 6 pages + references. How?
TODO - 1) Action item: qualify the CBP contribution
Bala is working on experiments -> 2) Action item: show that our model is SOTA, as one of its contributions
Done -> 3) Action item: use influencer/follower in the motivation as an example, but not everywhere after. 

Detailed comments and misc edits below:

Compare to other CBP methods: Dorsa Sadigh introduced the idea in RSS’16 (with IRL-based models), and Ed Schmerling did it with neural nets (conditional VAEs) in ICRA’18. 

Explain surprise in more detail.  One section claims that it predicts “surprise”, meaning situations where marginal predictions are different from conditional predictions. It does so by definition. Why is that useful though? 

Explain that the "Selecting Salient Agents" section is actually imitating a planner, so we are demonstrating what's useful for a planner. 
To show utility, you’d have to actually use these in planning and show that ignoring the agents with low mutual information does not affect the AV’s performance (either the plan, or, more ideally, the cost/reward of the resulting behavior when the ignored agents are actually present). 

Explain why we don't use joint models P(a,b), rather than having to train a conditional prediction model P(b|a). How can you justify conditional prediction? 

Results comments:

B is more of a sanity check that conditioning is helpful; Early fusion vs late fusion stuff — seems tangential/ distracts from the point 

C what’s the takeaway? Is this useful or purely informational or a sanity check on the score?

D 

Not sure what the term surprise refers to here, and what “surprising” interactions are. We throw it around at waymo but it’s not established in the robotics, HRI, and ML literature. It seems to be defined as KL divergence being high :)

Fig 4a the fact that what has highest mutual information has low to lowest delta wade, explained in the text as wade not being meaningful, seems to somewhat invalidate using it as a way to sanity check the score. 

4b seems to indicate that maybe the paper should have been about the KL divergence as a metric, or at least in equal parts with info gain. But the fact that it doesn’t have the problem that 4a has suggests that perhaps there is something wrong with Info gain not actually pointing at the kind of interactivity we care about.

E not sure how all of the sudden there is an AV, as the dataset described in the beginning mentioned “agents” (btw, waymo refers to humans as agents, but it’s not standard) — was there an AV in the data all along? Did it drive in manual? 

Need to motivate why you’d ignore agents for planning.

Other:

Need to change to active voice — you’re using passive voice too much which leads to reader fatigue.

==> deprecated/old_intro.tex <==
% MOVE TO RELWORK:
% Clearly, obtaining accurate predictions for other agents requires accounting for their interactions. There are a variety of existing approaches which attempt to do this task using relationship-based deep learning architectures such as transformers \cite{giuliari2020transformer}, or Graph Neural Networks (GNNs) \cite{casas2019spatially}, with positive results. 

% However, the field currently lacks a rigorous mathematical treatment of the notion of an interaction. We define interactions in the context of behavior prediction via an information-theoretic approach, and show how this treatment can provide key benefits when constructing behavior prediction models. 
% \textcolor{red}{Mathematical Details}
% Specifically, we use the \emph{mutual information} between the future trajectories of a pair of agents as an interactivity score that represents the potential for the two agents to have an unexpected interaction. %To compute an estimate of the mutual information between agent trajectories, we leverage state of the art BP models.


% \textcolor{red}{CBP}
% One important outcome of this work is the notion of a \emph{Conditional Behavior Prediction (CBP)} model. Typical behavior prediction systems are unconditional, and their outputs do not take the AV's plan into account \cite{bajcsy2020}. This imposes certain limitations on the system, as it encodes the assumption that human-driven cars will not react to the autonomous vehicle, often resulting in overly-cautious behaviors \cite{fisac2018probabilistically}. We leverage our work on interactions to develop a new approach to behavior prediction where predictions are conditioned on the planned trajectory of the AV.  
% We show that modeling the potential effect of the AV's behavior on other agents can greatly improve prediction accuracy, resulting in faster and safer AV behavior.


% \textcolor{red}{Importance of Autonomous driving}
% Autonomous driving is a key area of active research in the machine learning community. Autonomous vehicles have the potential to prevent accidents, save lives, reduce congestion, and empower those who are unable to drive themselves. It is also considered a gateway technology to the development of more general autonomous agents which can function freely within a chaotic human world. 
% %Most autonomous driving systems can be decomposed into three distinct components: Perception, Behavior Prediction, and Planning. Perception resolves sensor data into objects, BP predicts the future location of dynamic objects, and planner uses these predictions as constraints to chart a course for the AV.

% \textcolor{red}{Behavior Prediction }
% Behavior Prediction (BP) is a core component in modern AV systems. BP is the process of mapping past observations to a distribution over possible future agent trajectories. These predictions are crucial when creating a motion plan for the AV. BP is a complex and challenging task, as it requires jointly modelling a collection of unique human agents with unknown intent. Furthermore agent behavior is highly interactive, with each agent continuously modulating its actions based on the observed behavior of those around it. 

% \textcolor{red}{Importance of interactions}
% It is clear that obtaining accurate BPs requires us to account for these interactions in our model. There are a variety of existing approaches which attempt to do this using relationship-based deep learning architectures such as transformers or GNNs \cite{casas2019spatially, giuliari2020transformer}, with positive results. However, the field currently lacks a rigorous mathematical treatment of the notion of an interaction. We define interactions in the context of BP via an information theoretic approach, and show how these results can provide key benefits when constructing BP models. 
% \textcolor{red}{Mathematical Details}
% Specifically, we use the mutual information between the future trajectories of a pair of agents as an interactivity score that represents the potential of two agents to have a surprising interaction. %To compute an estimate of the mutual information between agent trajectories, we leverage state of the art BP models.

% \textcolor{red}{CBP}
% In particular, one important outcome of this work is the notion of a conditional behavior prediction model. Existing BP systems are unconditional, with the predicted behavior static during the planning phase \cite{bajcsy2020}. This imposes certain limitations on the system, as it encodes the assumption that human-driven cars will not react to the autonomous vehicle, often resulting in overly cautious behaviors \cite{fisac2018probabilistically}. We leverage our work on interactions to develop a new approach to BP where predictions are conditioned on the planned trajectory of the AV. We call this approach \emph{Conditional} behavior prediction (CBP). We show that predicting the effect of AV motion on agent behavior can greatly improve predictive accuracy, resulting in faster and safer AV behavior.

% \textcolor{red}{contributions}
% Our contributions can be summarized as follows: (1) We provide a problem-agnostic definition of agent interaction and a quantitative interactivity score. (2) We propose a unified architecture for conditional behavior prediction. (3) We demonstrate the utility of identifying interactions in real traffic scenarios.


%In traditional behavior prediction we estimate a distribution over future trajectories for each agent independently. This means that when we consider multiple agents in a scene, their BPs are often conflicting or inconsistent. More advanced approaches attempt to produce joint predictions which produce consistent predictions for all agents in a scene using models such as transformers or graph neural networks. We propose taking this a step further and conditioning our predictions 

%\textcolor{red}{Importance of CBP}
% On the road, an autonomous vehicle's action can affect the actions of other cars. Robot motion planning in the presence of humans is a well studied challenge.  Most planning approaches assume that human-driven cars will not react to the autonomous vehicle, often resulting in overly cautious behaviors \cite{fisac2018probabilistically}. Others approaches focus on planning using a cost function that combines efficiency of the trajectory and the inferred cost functions of human drivers \cite{sadigh2016planning}. In challenging scenarios, the autonomous car may need to balance the influence on other drivers with efficiency objectives. Predicting the effect of potential future plans on others can allow a planner to perform these trade-offs explicitly and make the resulting trajectories more efficient and safe.

% Another application could be focusing only on salient agents when simulating reactive policies for testing autonomous driving software.
% \textcolor{red}{Motivation 1) Anticipating situations of surprise. 2) Identifying interacting agents for high-fidelity prediction models/planning.}

% Interactive driving scenarios, such as lane changes, merges or unprotected turns, are some of the most challenging problems for autonomous driving. Planning in interactive scenarios requires accurately predicting the reactions of other agents to a particular future action. We develop end-to-end models for conditional behavior prediction (CBP) that take as an input a potential future trajectory for a vehicle, and predict the effect of this trajectory on other vehicles in the scene. 

%\textcolor{blue}{multi-modality of predictions, why MultiPath}
%A major challenge in driver behavior prediction is the inability to observe an agent's intention or goal. As a result, a drivers' behavior may appear multi-modal, with several possible actions being equally likely. We use the MultiPath architecture that explicitly predicts multi-modal distributions for the future trajectories of each agent \cite{chai2019multipath}.
%MultiPath is a one-shot long-horizon model so it allows us to capture longer-term correlations between agents’ futures. The interactivity score between two agents over a single time-step may be small, but only using one-shot long-horizon prediction models can we draw a more definitive conclusion. The long-horizon model also can capture second order effects in which the actions of one agent cause a chain reaction of influence, like sudden braking propagating several cars back. Therefore, the Conditional MultiPath \textcolor{red}{Let's define this properly first} model is unique in its ability to identify interactive situations. 



%\textcolor{blue}{related work in CBP/joint prediction}
%What-If Motion Prediction predicts the future trajectory for an agent conditioned on its nominal desired future trajectory \cite{khandelwal2020if}. Conditional MultiPath is not unique in its ability to perform multi-modal multi-agent behavior prediction, but it is uniquely suited for the use of its outputs for further analysis of driver interaction.


% Several state-of-the-art behavior prediction approaches also provide the ability to evaluate joint futures of multiple vehicles \cite{tang2019multiple, rhinehart2019precog, salzmann2020trajectron++, mangalam2020not, khandelwal2020if}. Like Conditional MultiPath, several other architectures allow the evaluation of conditional futures for a particular plan of the autonomous car. The Multiple Futures Prediction approach computes joint behavior predictions for multiple agents and also provides the ability to do hypothetical rollouts, but only limited evaluation is performed for this feature \cite{tang2019multiple}. PRECOG  provides a conditional query to the model via a latent space \cite{rhinehart2019precog}. The system must optimize over the latent vector to find the desired trajectory closest to the plan of the autonomous vehicle. Trajectron++ demonstrates the use of the ego future for improving behavior metrics on average, but does not consider conditioning on other vehicles \cite{salzmann2020trajectron++}. PECNet  infers possible goal locations for other agents and uses those to perform more accurate behavior prediction \cite{mangalam2020not}.



% \textcolor{blue}{The story from delta log likelihood, to KL divergence, to mutual information goes here.}



%\cite{kruse2013human}
% \textcolor{red}{Importance of Autonomous driving}
% Autonomous Vehicles (AVs) have the potential to prevent accidents, save lives, reduce congestion, and empower those who are unable to drive themselves. Autonomous driving is a key area of active research in the machine learning community and a gateway technology to the development of more general autonomous agents, which can function freely within a chaotic human world. 
%Most autonomous driving systems can be decomposed into three distinct components: Perception, Behavior Prediction, and Planning. Perception resolves sensor data into objects, BP predicts the future location of dynamic objects, and planner uses these predictions as constraints to chart a course for the AV.

% Another body of work seeks to learn a reward function of human agents via inverse reinforcement learning and use this reward to plan robot trajectories that optimize for both the robot's and humans objective \cite{ziebart2009planning, sadigh2016planning}. Recent work in the field seeks to predict the future trajectory of a human agent in proximity of a robot, and constrain the planning problem based on the predicted dynamic occupancy \cite{fisac2018probabilistically}. A Bayesian model of the future trajectory can allow the robot to plan more aggressive trajectories when the prediction uncertainty is low \cite{bajcsy2019scalable}. The predictions may be inaccurate if the intent of the human agent is unknown, so the robot may need to be robust to any possible future human trajectory \cite{bajcsy2020}. %Another work seeks to model the trajectories of the human and robot as Gaussian Processes and the model can be conditioned on the goal pose of the robot \cite{trautman2010unfreezing}.

% The biggest limitation of many of the approaches mentioned for human-aware control is the simplicity of the behavior prediction model. Real road traffic scenarios can include challenging interactions among dozens of agents, such as drivers, cyclists and pedestrians, and the problem of driver behavior prediction is an emerging field of research. Several state-of-the-art behavior prediction approaches provide the ability to evaluate joint futures of multiple vehicles \cite{tang2019multiple, rhinehart2019precog, salzmann2020trajectron++, mangalam2020not, khandelwal2020if}. Furthermore, several of these architectures allow the evaluation of conditional futures for a particular plan of the autonomous car. The Multiple Futures Prediction approach computes joint behavior predictions for multiple agents and also provides the ability to do hypothetical rollouts, but only limited evaluation is performed for this feature \cite{tang2019multiple}. PRECOG  provides a potential future AV trajectory to the model via a latent space representation \cite{rhinehart2019precog}. The system must optimize over the latent vector to find the desired trajectory closest to the plan of the autonomous vehicle. Trajectron++ demonstrates the use of the ego future for improving behavior metrics on average, but does not consider conditioning on other vehicles \cite{salzmann2020trajectron++}. PECNet infers possible goal locations for other agents and uses those to perform more accurate behavior prediction \cite{mangalam2020not}.
% Our approach to estimating agent interactivity scores could potentially be used with any model that enables the evaluation of conditional predictions.




